Sandslash: A Two-Level Framework for Efficient Graph Pattern Mining

Graph pattern mining (GPM) is used in diverse application areas including social network analysis, bioinformatics, and chemical engineering. Existing GPM frameworks either provide high-level interfaces for productivity at the cost of expressiveness or provide low-level interfaces that can express a wide variety of GPM algorithms at the cost of increased programming complexity. Moreover, existing systems lack the flexibility to explore combinations of optimizations to achieve performance competitive with hand-optimized applications. We present Sandslash, an in-memory Graph Pattern Mining (GPM) framework that uses a novel programming interface to support productive, expressive, and efficient GPM on large graphs. Sandslash provides a high-level API that needs only a specification of the GPM problem, and it implements fast subgraph enumeration, provides efficient data structures, and applies high-level optimizations automatically. To achieve performance competitive with expert-optimized implementations, Sandslash also provides a low-level API that allows users to express algorithm-specific optimizations. This enables Sandslash to support both high-productivity and high-efficiency without losing expressiveness. We evaluate Sandslash on shared-memory machines using five GPM applications and a wide range of large real-world graphs. Experimental results demonstrate that applications written using Sandslash high-level or low-level API outperforms state-of-the-art GPM systems AutoMine, Pangolin, and Peregrine on average by 13.8x, 7.9x, and 5.4x, respectively. We also show that these Sandslash applications outperform expert-optimized GPM implementations by 2.3x on average with less programming effort.

==> sections/design.tex <==
%\begin{figure}[t]
%	\begin{center}
%		\includegraphics[width=0.49\textwidth]{figures/bfs-dfs.pdf}
%		\caption{BFS vs. DFS exploration of the subgraph tree.}
%		\label{fig:bfs-dfs}
%	\end{center}
%\end{figure}

%\begin{figure}[t]
%	\begin{center}
%		\includegraphics[width=0.48\textwidth]{figures/enum.pdf}
%		\caption{An example of embedding enumeration.
%			The gray embeddings are non-canonical automorphisms.}
%		\label{fig:enum}
%	\end{center}
%\end{figure}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{1,1,1}
\lstdefinestyle{mystyle}{
	backgroundcolor=\color{backcolour},
	commentstyle=\color{codegreen},
	keywordstyle=\color{blue},
	numberstyle=\tiny\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\footnotesize\ttfamily,
	breakatwhitespace=false,
	breaklines=true,
	captionpos=b,
	keepspaces=true,
	numbers=left,
	numbersep=5pt,
	showspaces=false,
	showstringspaces=false,
	showtabs=false,
	tabsize=2
}
\lstset{style=mystyle}
\lstset{aboveskip=0pt,belowskip=-5pt}

\section{Overview of Sandslash}\label{sect:design}


\begin{algorithm}[t]
	\small
	\caption{DFS Execution Model (vertex-induced)}
	\label{alg:engine}
	\begin{algorithmic}[1]
		\Procedure{MineEngine}{$G$($V$,$E$), MAX\_SIZE}
		\For{each edge $e \in G$ in parallel}
			%\State \Call{Init}{$e$, $emb\_list$} \Comment{insert single-edge embedding}
			\State $level \leftarrow 1$
			\State $history[0] \leftarrow e.src$
			%\State \Call{updateCode}{$0$, $e.src$}
			\State insert $e.dst$ to $frontier(1)$
			\State \Call{DfsMine}{$level$, $history$, $frontier$}
		\EndFor
		\EndProcedure
		
		\item[]
		
		\Procedure{DfsMine}{$level$, $history$, $frontier$}
		%\State \Call{\textcolor{blue}{Reduce}}{$emb\_list$, $p\_map$}
		%\State \Call{\textcolor{blue}{Filter}}{$emb\_list$, $p\_map$}
		\If{$level =$ MAX\_SIZE - 1}
			\State \Call{\textcolor{blue}{Reduce}}{$level$, $history$, $frontier$}
			\State \Return
		\EndIf
		\For{each $v$ in $frontier(level)$}
			\State $history[level] \leftarrow v$
			\State \Call{\textcolor{blue}{Extend}}{$level$, $history$, $frontier$}
			\State \Call{DfsMine}{$level+1$, $history$, $frontier$}
			%\State \Call{resumeCode}{$level$, $v$}
			\State $history$.pop()
		\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
	\small
	\caption{Extend Phase (vertex-induced)}
	\label{alg:extend}
	\begin{algorithmic}[1]
		%\Procedure{Extend}{$level$, $emb$, $emb\_list$}
		\Procedure{Extend}{$level$, $emb$, $frontier$}
		%\State \Call{\textcolor{blue}{updateCode}}{$level$, $emb$.getLastVertex()}
		\For{each vertex $v$ in $emb$}
			\If{\Call{\textcolor{blue}{toExtend}}{$emb$, $v$} = $true$}
				\For{each vertex $u$ in $adj(v)$}
					\If{\Call{\textcolor{blue}{toAdd}}{$emb$, $u$} = $true$}
						%\State insert $u$ to $emb\_list(level+1)$
						\State insert $u$ to $frontier(level+1)$
					\EndIf
				\EndFor
			\EndIf
		\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
\small
\caption{Reduce Phase (vertex-induced)}
\label{alg:reduce}
\begin{algorithmic}[1]
	\Procedure{Reduce}{$level$, $history$, $frontier$}
	\State $p\_map \leftarrow \emptyset$ \Comment{clear the pattern map}
	\For{each $v$ in $frontier(level)$}
		\State EmbTy $emb \leftarrow  history[level] \cap v$
	%\State \Call{\textcolor{blue}{updateCode}}{$level$, $emb$.getLastVertex()}
	%\For{each vertex $v$ in $emb$}
	%	\If{\Call{\textcolor{blue}{toExtend}}{$emb$, $v$} = $true$}
	%		\For{each vertex $u$ in $adj(v)$}
	%			\If{\Call{\textcolor{blue}{toAdd}}{$emb$, $u$} = $true$}
					\State Pattern $pt \leftarrow $ \Call{\textcolor{blue}{getPattern}}{$emb$}
					\State Support $sp \leftarrow $ \Call{\textcolor{blue}{getSupport}}{$emb$}
					\State \Call{\textcolor{blue}{Aggregate}}{$p\_map$[$pt$], $sp$}
	%			\EndIf
	%		\EndFor
	%	\EndIf
	\EndFor
	\EndProcedure
\end{algorithmic}
\end{algorithm}




\begin{lstlisting}[float=tp,floatplacement=b,label={lst:api},language=C++,abovecaptionskip=0pt,caption={User-defined functions.}]
bool toExtend(EmbTy emb, Vertex v);
bool toAdd(EmbTy emb, Vertex u)
bool toAdd(EmbTy emb, Edge e)
Pattern getPattern(EmbTy emb)
Support getSupport(EmbTy emb)
Support Aggregate(Support s1, Support s2)
bool toDiscard(EmbTy emb);
bool toDiscard(Pattern pt);
\end{lstlisting}
\iffalse
void buildLocalGraph();
void updateLocalGraph();
void post-process();
\fi

%\subsection{Two-level Programming Interface}



One way around this problem is to provide a lower-level API that gives
the user more control over the search. In particular, the API should permit
the user to prune the search selectively based on problem and pattern specific insights such as the sub-clique property for k-CL.

Existing systems support either a high-level or a low-level API, giving up either on
performance or productivity. Sandslash attempts to get the best of both worlds by
permitting the user to program using a high-level API but provides a low-level API as well to permit the user to control the search process as needed. When the user wants to find a explicit pattern such as a triangle or 4-cycle, the only thing required is to provide the pattern as a graph to the system. Sandslash takes the pattern and generates a parallel implementation automatically. When user is not satisfied with the performance of the automatically generated solution or the pattern(s) of interest are difficult to specify explicitly (as in FSM), the low-level API functions can be used \emph{selectively} to control the search process.





==> sections/engine.tex <==

% To understand what these API functions do, it is necessary to
% understand some of the internals of Sandslash. \cref{sec:internals}
% introduce how the execution engine exposes API functions.
% The rest subsections describe low-level optimizations in \cref{tab:opt}
% (right) and shows how they can be implemented using the API functions.

\begin{algorithm}[t]
	\footnotesize
	\caption{\small Execution Engine (vertex-induced; edge-parallel)}
	\label{alg:engine}
	\begin{algorithmic}[1]
		\Procedure{MineEngine}{$G$($V$,$E$), $k$}\Comment{$k$ is pattern size}
		\For{each edge $e \in G$ in parallel} \Comment{edge parallel}
			\State $level \leftarrow 1$; $history \leftarrow queue()$; $frontier \leftarrow map()$
			\State $history$.push($e.src$) \Comment{$v_0$ in level 0}
			\State $frontier[level]$.insert($e.dst$) \Comment{$v_1$ in level 1}
			\State \Call{DfsMine}{$level$, $history$, $frontier$}
		\EndFor
		\EndProcedure
		
		\item[]
		
		\Procedure{DfsMine}{$level$, $history$, $frontier$}
		\If{$level = k-1$} \Comment{stop extension}
			\State \Call{\textcolor{blue}{Aggregate}}{$level$, $history$, $frontier$}\Comment{support reduction}
			\State \Return
		\EndIf
		\For{each $v$ in $frontier[level]$}
			%\State $history[level] \leftarrow v$
			\State $history$.push($v$)
			\State \Call{\textcolor{blue}{Extend}}{$level$, $history$, $frontier$}\Comment{vertex extension}
			\State \Call{DfsMine}{$level+1$, $history$, $frontier$}\Comment{go to next level}
			\State $frontier[level+1] \leftarrow \{\}$
			\State $history$.pop()
		\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}



% \subsection{Sandslash Internals for Low-level API}\label{sec:internals}

% We introduce how the API functions are exposed to the user in the
% context of the DFS execution engine in \cref{alg:engine}.
% \cref{alg:extend} shows its \textproc{Extend} phase. Each vertex in
% the current embedding (line 2) is considered for extension with one
% of its neighbors (line 4). If the user only wants to extend a subset
% of the vertices in the embedding, the {\tt\small toExtend} function
% (line 3) can be used to select them. For the new vertex $u$ extended
% from $v$, the user can apply a automorphism check using the {\tt\small
% toAdd} function (line 5). Canonical embeddings are inserted into
% the embedding list (line 6). However, to perform a non-canonical
% enumeration, the user can just re-implement the \texttt{\small
% toAdd} function to replace the default check. In summary, the user
% can use {\tt\small toExtend}  and {\tt\small toAdd} to prune the
% search space.

% \cref{alg:reduce} shows the \textproc{Aggregate} phase. In this stage,
% the input is the embedding list and the output is a pattern-map.
% The pattern-map contains the support for each pattern of interest.
% %For example, in FSM the map maintains the domain support for each
% %frequent pattern, while in TC the map is a single accumulator for triangle.
% To compute this map, it takes each embedding (line 3 \& 4),
% finds its pattern using {\tt\small getPattern} (line 5), gets its
% support using {\tt\small getSupport} (line 6), and aggregates the
% support to the map (line 7). {\tt\small getPattern} can be
% implemented by applying a GI test, however, the user can
% reimplement it with a customized method to identify pattern.
% As for the other functions in \cref{lst:lo-api},
% {\tt\small localReduce} replaces {\tt\small reduce} at line 7
% when local counting is used by the user.
% {\tt\small initLG} and {\tt\small updateLG} are invoked before
% and after the extension at each level respectively.
% %at line 6 of \cref{alg:engine}, while  happens after each
% %extension at line 13 of \cref{alg:engine}.

% \begin{algorithm}[t]
% \footnotesize
% \caption{\small Extend Phase (vertex-induced)}
% \label{alg:extend}
% 	\begin{algorithmic}[1]
% 		%\Procedure{Extend}{$level$, $emb$, $emb\_list$}
% 		\Procedure{Extend}{$level$, $emb$, $frontier$}
% 		%\State \Call{\textcolor{blue}{updateCode}}{$level$, $emb$.getLastVertex()}
% 		\For{each vertex $v$ in $emb$}
% 			\If{\Call{\textcolor{blue}{toExtend}}{$emb$, $v$} = $true$}
% 				\For{each vertex $u$ in $adj(v)$}
% 					\If{\Call{\textcolor{blue}{toAdd}}{$emb$, $u$} = $false$}
% 						%\State insert $u$ to $emb\_list(level+1)$
% 						\State $frontier[level+1]$.insert($u$)
% 					\EndIf
% 				\EndFor
% 			\EndIf
% 		\EndFor
% 		\EndProcedure
% 	\end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[t]
% \footnotesize
% \caption{\small Aggregate Phase (vertex-induced)}
% \label{alg:reduce}
% \begin{algorithmic}[1]
% 	\Procedure{Aggregate}{$level$, $history$, $frontier$}
% 	\State $p\_map \leftarrow \emptyset$ \Comment{clear the pattern map}
% 	\For{each $v$ in $frontier[level]$}
% 		\State Embbedding $emb \leftarrow  history \cap v$ \Comment{candidate embedding}
% 		\State Pattern $pt \leftarrow $ \Call{\textcolor{blue}{getPattern}}{$emb$}
% 		\State Support $sp \leftarrow $ \Call{\textcolor{blue}{getSupport}}{$emb$}
% 		\State \Call{\textcolor{blue}{reduce}}{$pt$, $p\_map$[$pt$], $sp$} \Comment{do reduction}
% 	\EndFor
% 	\EndProcedure
% \end{algorithmic}
% \end{algorithm}

==> sections/impl.tex <==
\section{Low-level API}\label{sect:impl}

%\begin{figure}[t]
%	\begin{center}
%		\includegraphics[width=0.49\textwidth]{figures/bfs-dfs.pdf}
%		\caption{BFS vs. DFS exploration of the subgraph tree.}
%		\label{fig:bfs-dfs}
%	\end{center}
%\end{figure}

%\begin{figure}[t]
%	\begin{center}
%		\includegraphics[width=0.48\textwidth]{figures/enum.pdf}
%		\caption{An example of embedding enumeration.
%			The gray embeddings are non-canonical automorphisms.}
%		\label{fig:enum}
%	\end{center}
%\end{figure}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{1,1,1}
\lstdefinestyle{mystyle}{
	backgroundcolor=\color{backcolour},
	commentstyle=\color{codegreen},
	keywordstyle=\color{blue},
	numberstyle=\tiny\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\footnotesize\ttfamily,
	breakatwhitespace=false,
	breaklines=true,
	captionpos=b,
	keepspaces=true,
	numbers=left,
	numbersep=5pt,
	showspaces=false,
	showstringspaces=false,
	showtabs=false,
	tabsize=2
}
\lstset{style=mystyle}
\lstset{aboveskip=0pt,belowskip=-5pt}

\section{Overview of Sandslash}\label{sect:design}


\begin{algorithm}[t]
	\small
	\caption{DFS Execution Model (vertex-induced)}
	\label{alg:engine}
	\begin{algorithmic}[1]
		\Procedure{MineEngine}{$G$($V$,$E$), MAX\_SIZE}
		\For{each edge $e \in G$ in parallel}
			%\State \Call{Init}{$e$, $emb\_list$} \Comment{insert single-edge embedding}
			\State $level \leftarrow 1$
			\State $history[0] \leftarrow e.src$
			%\State \Call{updateCode}{$0$, $e.src$}
			\State insert $e.dst$ to $frontier(1)$
			\State \Call{DfsMine}{$level$, $history$, $frontier$}
		\EndFor
		\EndProcedure
		
		\item[]
		
		\Procedure{DfsMine}{$level$, $history$, $frontier$}
		%\State \Call{\textcolor{blue}{Reduce}}{$emb\_list$, $p\_map$}
		%\State \Call{\textcolor{blue}{Filter}}{$emb\_list$, $p\_map$}
		\If{$level =$ MAX\_SIZE - 1}
			\State \Call{\textcolor{blue}{Reduce}}{$level$, $history$, $frontier$}
			\State \Return
		\EndIf
		\For{each $v$ in $frontier(level)$}
			\State $history[level] \leftarrow v$
			\State \Call{\textcolor{blue}{Extend}}{$level$, $history$, $frontier$}
			\State \Call{DfsMine}{$level+1$, $history$, $frontier$}
			%\State \Call{resumeCode}{$level$, $v$}
			\State $history$.pop()
		\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
	\small
	\caption{Extend Phase (vertex-induced)}
	\label{alg:extend}
	\begin{algorithmic}[1]
		%\Procedure{Extend}{$level$, $emb$, $emb\_list$}
		\Procedure{Extend}{$level$, $emb$, $frontier$}
		%\State \Call{\textcolor{blue}{updateCode}}{$level$, $emb$.getLastVertex()}
		\For{each vertex $v$ in $emb$}
			\If{\Call{\textcolor{blue}{toExtend}}{$emb$, $v$} = $true$}
				\For{each vertex $u$ in $adj(v)$}
					\If{\Call{\textcolor{blue}{toAdd}}{$emb$, $u$} = $true$}
						%\State insert $u$ to $emb\_list(level+1)$
						\State insert $u$ to $frontier(level+1)$
					\EndIf
				\EndFor
			\EndIf
		\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
\small
\caption{Reduce Phase (vertex-induced)}
\label{alg:reduce}
\begin{algorithmic}[1]
	\Procedure{Reduce}{$level$, $history$, $frontier$}
	\State $p\_map \leftarrow \emptyset$ \Comment{clear the pattern map}
	\For{each $v$ in $frontier(level)$}
		\State EmbTy $emb \leftarrow  history[level] \cap v$
	%\State \Call{\textcolor{blue}{updateCode}}{$level$, $emb$.getLastVertex()}
	%\For{each vertex $v$ in $emb$}
	%	\If{\Call{\textcolor{blue}{toExtend}}{$emb$, $v$} = $true$}
	%		\For{each vertex $u$ in $adj(v)$}
	%			\If{\Call{\textcolor{blue}{toAdd}}{$emb$, $u$} = $true$}
					\State Pattern $pt \leftarrow $ \Call{\textcolor{blue}{getPattern}}{$emb$}
					\State Support $sp \leftarrow $ \Call{\textcolor{blue}{getSupport}}{$emb$}
					\State \Call{\textcolor{blue}{Aggregate}}{$p\_map$[$pt$], $sp$}
	%			\EndIf
	%		\EndFor
	%	\EndIf
	\EndFor
	\EndProcedure
\end{algorithmic}
\end{algorithm}




\begin{lstlisting}[float=tp,floatplacement=b,label={lst:api},language=C++,abovecaptionskip=0pt,caption={User-defined functions.}]
bool toExtend(EmbTy emb, Vertex v);
bool toAdd(EmbTy emb, Vertex u)
bool toAdd(EmbTy emb, Edge e)
Pattern getPattern(EmbTy emb)
Support getSupport(EmbTy emb)
Support Aggregate(Support s1, Support s2)
bool toDiscard(EmbTy emb);
bool toDiscard(Pattern pt);
\end{lstlisting}
\iffalse
void buildLocalGraph();
void updateLocalGraph();
void post-process();
\fi

%\subsection{Two-level Programming Interface}



One way around this problem is to provide a lower-level API that gives
the user more control over the search. In particular, the API should permit
the user to prune the search selectively based on problem and pattern specific insights such as the sub-clique property for k-CL.

Existing systems support either a high-level or a low-level API, giving up either on
performance or productivity. Sandslash attempts to get the best of both worlds by
permitting the user to program using a high-level API but provides a low-level API as well to permit the user to control the search process as needed. When the user wants to find a explicit pattern such as a triangle or 4-cycle, the only thing required is to provide the pattern as a graph to the system. Sandslash takes the pattern and generates a parallel implementation automatically. When user is not satisfied with the performance of the automatically generated solution or the pattern(s) of interest are difficult to specify explicitly (as in FSM), the low-level API functions can be used \emph{selectively} to control the search process.

\subsection{Execution Model}


Classified by the over-counting property, there are two types of mining algorithms.
The first category is \emph{canonical enumeration}, which only enumerate canonical
embeddings without over-counting.
For example, people uses orientation for TC (similar for $k$-CL) to pre-define
a search ordering. In this case any triangle in the input graph will be enumerated
only once. Another example is Arabesque, which uses a generic automorphism check
algorithm to select canonical embeddings and discard non-canonical ones on-the-fly.
Either static (orientation) or dynamic (generic automorphism check) approach
guarantees that each embedding is enumerated only once.
The second category is \emph{non-canonical enumeration} which over-counts
the embeddings and does post-processing to fix the output.
For example, each triangle can be counted for three times
by starting from any of its three edges. The total count is
divided by 3 afterwards to get the correct number of triangles.

Sandslash supports both canonical and non-canonical enumeration
in a unified execution model. As shown in \cref{alg:engine},
a parallel DFS walk starts from each edge (line 2). In depth 1,
the edge is inserted into the embedding list (line 4 \& 5) and the
engine invokes a recursive sub-procedure \textproc{DfsMine} (line 6).
In \textproc{DfsMine}, if it reaches the user-defined maximum size
$k$ (line 8), it performs a reduction on the embeddings (line 9).
Otherwise, it iterates over each element in the frontier (line 11),
does a extension (line 13), and goes to the next level (line 14).

\cref{alg:extend} shows the \textproc{Extend} phase.
In this stage, each vertex in the embedding (line 2) is considered
to be extended with one of its neighbors (line 4). If the user
only wants to extend a subset of the vertices in the embedding,
the \texttt{\small toExtend} function (line 3) can be used to
select them. For the new vertex $u$ extended from $v$, the user can
apply canonical test using the \texttt{\small toAdd} function (line 5).
Only canonical embeddings can pass the test and be inserted into
the embedding list (line 6).
However, to perform a non-canonical enumeration, the user just
needs to re-implement the \texttt{\small toAdd} function without
canonical test.

\cref{alg:reduce} shows the \textproc{Reduce} phase. In this stage,
the input is the embedding list, and the output is a pattern-map
which contains the statistical information that the user needs.
For example, in FSM this map maintains the support for each pattern,
while in TC this map is a single accumulator. To compute this map,
it takes each embedding in the embedding list (line 3 \& 4),
finds its pattern using \textproc{getPattern} (line 5), gets its
support using \textproc{getSupport} (line 6), and aggregates the
support to the pattern map (line 7).



\begin{lstlisting}[float=tp,floatplacement=tbp,label={lst:kcl},language=C++,abovecaptionskip=0pt,caption=Clique Listing (baseline).]
bool toAdd(EmbTy emb, Vertex v) {
	return is_auto_canonical(emb, v) && is_all_connected(v, emb);
}
\end{lstlisting}

\begin{lstlisting}[float=tp,floatplacement=tbp,label={lst:kcl-opt},language=C++,abovecaptionskip=0pt,caption=Clique Listing (optimized).]
#define USE_DAG
bool toExtend(EmbTy emb, Vertex v) {
	// only extend the last vertex
	return v.idx == emb.size() - 1;
}
bool toAdd(EmbTy emb, Vertex v) {
	uint8 level = emb.size() - 1;
	return get_qcode(v) == pow(2,level)-1;
}
\end{lstlisting}

\iffalse
\begin{lstlisting}[float=tp,floatplacement=tbp,label={lst:kcl},language=C++,abovecaptionskip=0pt,caption=Clique Listing (qcode compressed).]
bool toAdd(EmbTy emb, Vertex v) {
	return get_qcode(v) == emb.size();
}
void updateCode(uint8 level, Vertex v) {
	for (each u : adj(v))
		if (get_qcode(u) == level)
			set_qcode(u, level+1);
}
void resumeCode(uint8 level, Vertex v) {
	for (each u : adj(v))
		if (get_qcode(u) == level+1)
			set_qcode(u, level);
}
\end{lstlisting}
\fi

\begin{lstlisting}[float=tp,floatplacement=tbp,label={lst:kcl},language=C++,abovecaptionskip=0pt,caption=Motif Listing (baseline).]
bool toExtend(EmbTy emb, Vertex v) {
	return true;
}
bool toAdd(EmbTy emb, Vertex v) {
	return is_auto_canonical(emb, v);
}
Pattern getPattern(EmbTy emb) {
	return get_iso_canonical(emb);
}
\end{lstlisting}

\begin{lstlisting}[float=tp,floatplacement=tbp,label={lst:kcl},language=C++,abovecaptionskip=0pt,caption=Motif Listing (optimized).]
Pattern getPattern(EmbTy emb) {
	uint8 level = emb.size() - 1;
	Vertex v = emb.getLastVertex();
	Ccode p_code = emb.get_pcode();
	Ccode q_code = get_qcode(v);
	if (level == 1) { // 3-motif
		if (c_code=='11') return TRI;
		else return WEDGE;
	} else (level == 2) { // 4-motif
		...
	} else return getIsoCanonical(emb);
}
\end{lstlisting}

\iffalse
void updateCode(uint8 level, Vertex v) {
	for (each u : adj(v))
	set_qcode(v, get_qcode(v)+(1<<level));
}

void resumeCode(uint8 level, Vertex v) {
	for (each u : adj(v))
	set_qcode(v, get_qcode(v)-(1<<level));
}

if (p_code == '111') {
	if (c_code=='111') return 4CLIQUE;
	else if (c_code=='110' or '101' or '011')
	return DIAMOND;
	else return TAILED_TRI;
} else if (p_code=='110') {
	if (c_code=='111') return DIAMOND;
	else if (c_code=='011') return 4CYCLE;
	else if (c_code=='100') return 3STAR;
	else if (c_code=='110' or '101')
	return TAILED_TRI;
	else return 3CHAIN;
} else { // p_code=='101'
	if (c_code=='111') return DIAMOND;
	else if (c_code=='101') return 4CYCLE;
	else if (c_code=='010') return 3STAR;
	else if (c_code=='110' or '011')
	return TAILED_TRI;
	else return 3CHAIN;
}
\fi

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.36\textwidth]{figures/diamond.pdf}
		\caption{An example of pattern identification for diamond.}
		\label{fig:diamond}
	\end{center}
\end{figure}


\cref{lst:api} lists the API functions provided by Sandslash.
The interface is mostly the same for BFS and DFS exploration,
except that for pattern-wise filtering (e.g needed bt FSM),
the \texttt{\small toDiscard} function accepts an embedding in
the BFS mode but a pattern in the DFS mode.
\todo{describe API}





\subsection{Avoiding Redundant Computation with PQ-Coding}\label{subsect:pq-code}
To identify the structure of a given embedding,
a common operation is to check connectivity among the vertices
in the embedding. Connectivity check is computationally
expensive because it requires searching the neighbor set,
which could be $O(E)$ for high-degree vertices in a power-law graph.
More importantly, in each level this connectivity needs to be
computed repeatedly, which leads to a huge amount of redundant
computation. For example, when enumerating triangles
for an edge $e=(u,v)$, an intersection of $u$ and $v$'s
neighbor set is computed to get the third vertices $w$,
i.e. $w \in N(u)\cap N(v)$. All vertices that are
connected to both $u$ and $v$ are computed. However,
when it comes to the next level, for each triangle
$t=(u,v,w)$, we need to check whether the fourth
vertex $x$ is connected to $u$, $v$ and $w$, i.e.
$x \in N(u)\cap N(v) \cap N(w)$. Note that $N(u)\cap N(v)$
is already computed in the previous level, which is
a redundant computation.

\input{sections/tbl_opt}

To avoid redundant computation, we need to memorize the
computed connectivity information. This information is
encoded using connectivity code.
At depth $d$ in the mining process, there is a history
of size $d+1$ that contains the current embedding
$H$=<$v_{0}$, $v_{1}$,$\dots$, $v_{d}$>. For any specific history,
there is a prefix-code (\texttt{p-code}) associated with it.
The \texttt{p-code} is a connectivity code that encodes
the connectivity information among vertices in $H$.
Extending vertices in $H$ can generate the frontier with
$n$ vertices $F$=\{$u_{0}$,$u_{1}$,$\dots$, $u_{n}$\}.
Concatenating $H$ with each element $u_{i}$
($i=0,1,\dots,n$) in $F$ gives us a new embedding
$Emb_{i}$=<$v_{0}$, $v_{1}$,$\dots$, $v_{d}$, $u_{i}$>.
Each vertex $v \in V$ is associated with a query
code (\texttt{q-code}).
The \texttt{q-code} is a connectivity code that encodes the
connectivity information between $v$ and all vertices in $H$.
To get the connectivity information of $u_{i}$ with any vertex in
$H$, we only need to query its \texttt{q-code} using its vertex id.
With \texttt{p-code} of $H$ and \texttt{q-code} of $u_{i}$,
we can identify the structure of $Emb_{i}$.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.49\textwidth]{figures/pq-code.pdf}
		\caption{An example of updating p-code and q-code.}
		\label{fig:pq-code}
	\end{center}
\end{figure}

\cref{fig:pq-code} shows an example of how p-code and q-code are
updated. In the beginning, p-code and q-code are initialized to 0.
Assume that it starts from the edge ($v_{1}$, $v_{2}$). Taking
$v_{1}$, we set the q-code of all the $v_{1}$' neighbor except
$v_{2}$. And the current p-code is `1' indicating $v_{2}$ is
connected to $v_{1}$. Then taking $v_{2}$, we set the q-code
of all the $v_{2}$' neighbor except $v_{1}$. When we add one more
vertex $v_{3}$ to the embedding, by checking $v_{3}$'s q-code,
we know that $v_{3}$ is connected to both $v_{1}$ and $v_{2}$,
which indicates that embedding <$v_{1}$, $v_{2}$, $v_{3}$>
is a triangle (p-code updated to `111').
Next it updates the q-code of all the $v_{3}$' neighbor.
Again, when another new vertex $v_{4}$ is added, by checking
$v_{4}$'s q-code, we know that $v_{4}$ is connected to $v_{2}$,
but not $v_{1}$ and $v_{3}$. Given the history embedding is a
triangle (by checking p-code), we know that the new embedding
is a tailed-triangle (p-code set to `111010').


\subsection{Support for Local Counting}\label{subsect:formula}
The major advantage of non-canonical enumeration is that the
local counts (e.g. the local count of triangles incident to
each edge) can be accumulated for each independent DFS walk.
These counts then can be used for calculating the counts
of other patterns without enumerating them at all.
For example, in 3-motif counting,
once $C_{tri}$ of an edge $e$: $(src, dst)$ is obtained,
$C_{wdg}$ can be computed with this formula:
$C_{wdg} = (deg_{src} - C_{tri} - 1) + (deg_{dst} - C_{tri} - 1)$,
where $deg_{src}$ and $deg_{dst}$ are the degree of the source
and destination vertex. \cref{fig:formula-example} shows an
example of 3-motif counting. Given $C_{wdg} \gg C_{tri}$,
avoiding enumerating all the wedges at the cost of
over-counting triangles (for three times) is a reasonable tradeoff.
This approach has already been extended to 4-MC~\cite{PGD} and 5-MC~\cite{ESCAPE}.

Sandslash supports non-canonical enumeration by simply implement
the \texttt{\small toAdd} function. This enables the
formula-based local counting approach for multi-pattern mining.
The user provides the patterns that needs to be enumerated,
as well as the formulas to compute the count of other patterns
in the post-processing API function (not listed in \cref{lst:api}).

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.25\textwidth]{figures/formula-example.pdf}
		\caption{An example of local counting.
			Given the local triangle count of edge $e$ is $C_{tri}=2$,
			and $deg_{u}=4, deg_{v}=5$, we can get $C_{wdg}=(4-2-1)+(5-2-1)=3$.}
		\label{fig:formula-example}
	\end{center}
\end{figure}

\subsection{Support for Local Graph Shrinking}\label{subsect:shrink}
For some special patterns the search area $S$ in the graph from each
edge is confined in a small set and shrinks as the DFS go deeper.
For example to find $k$-cliques incident to an edge $e$: $(src, dst)$,
we only need to search the subgraph induced by the common neighbors
of vertex $src$ and $dst$, i.e. $S = N(src) \cap N(dst)$, where $N(v)$
is the set of neighbors of vertex $v$. Besides, each time a new vertex
$u$ is added into the embedding, the search area is shrank with
$S_{i} = S_{i-1} \cap N(u)$, where $S_{i}$ is the search area in level
$i$ of the depth-first search. Therefore, to further reduce the search
space for special patterns, an optimization, \emph{local graph shrinking},
is introduced to confine the search area in the graph.

To enable local graph shrinking in Sandslash,
the user needs to specify how to initialize (\texttt{\small initLocalGraph})
and update (\texttt{\small updateLocalGraph}) the local graph in each level,
e.g. perform intersection in the case of $k$-CL.
If the user implements these API functions, a local graph instead
of the original global graph is used to get the neighborhood
information during extension. Apparently, searching over this
shrinking local graph is much less expensive than searching
over the original global graph.

\subsection{Other Optimization}\label{subsect:other}
\emph{Eager pruning}.
For some applications, such as TC and $k$-CL~\cite{KClique},
duplicate embeddings can be detected eagerly before
extending current embeddings. In $k$-CL, for any embedding
it is safe to only extend one of the vertices.
Assume that an embedding $Emb_{i-1}$=<$v_{1}$, $v_{2}$, $\dots$, $v_{i-1}$> is
extended to a new embedding $Emb_{i}$=<$v_{1}$, $v_{2}$, $\dots$, $v_{i-1}$, $u$>
by adding vertex $u$. If $Emb_{i}$ is an $i$-clique,
then by definition $u$ is a neighbor of $v_{1}$, $v_{2}$, $\dots$, and $v_{i-1}$.
This indicates that extending any vertex in $Emb_{i-1}$
will get $u$. In this case it is safe to only extend $v_{i-1}$ and
still guarantee completeness. If $Emb_{i}$ is not an $i$-clique,
then there is no need to enumerate it since it will definitely
not grow into a $k$-clique.
In Sandslash, as shown in Listing~\ref{lst:kcl-opt},
only the last vertex of the current embedding needs to be extended.
This aggressive pruning significantly reduces the search space.
If the pattern is given by the user, e.g. a triangle,
by simply checking the connectivity code of the pattern, Sandslash
detects the condition and enables this optimization automatically.

\emph{Orientation}.
This technique has been adopted in TC~\cite{Schank}, $k$-CL~\cite{KClique},
and $4,5$-MC~\cite{ESCAPE}. The idea is to establish a total ordering among vertices,
which converts the input graph into a Directed Acyclic Graph (DAG).
The search is then done over this DAG instead of the original input graph,
which substantially reduces the search space. In Sandslash,
the ordering among vertices is established based on their degrees:
each edge points towards the vertex with higher degree.
When there is a tie, the edge points to the vertex with larger vertex ID.
Other orderings, e.g core value based ordering, can be included in the future.

Customized pattern classification

Degree filtering

\section{Implementation}\label{sect:impl}
\subsection{Pattern Reduction in DFS Mode}
Depending on the definition of support, different mining
applications may need different computation for pattern reduction.
For all the vertex-induced application considered in this paper,
the reduction is simply accumulating embedding count(s).
This can be done by different threads independently,
and then local counts are combined afterwards to get the global count.
However, applications such as FSM requires pattern filtering at every level,
which discard all the embeddings of a pattern whose
support $\sigma$ is below a threshold $\sigma_{min}$.
In this case, embeddings in the same level have to be
gathered together to compute $\sigma$, which requires
level-wise synchronization among these embeddings.
In the BFS mode, the mining process runs in a bulk synchronous
parallel (BSP) fashion. All the embeddings are inherently
synchronized level by level. However, in DFS mode, each
thread does an independent DFS walk, and at a specific
moment, different threads can be at different level.
In this case, there is no way to gather embeddings for
each pattern.

To support pattern reduction in DFS mode, we introduce
\emph{embedding gathering} in the \textproc{Extend} phase.
Each pattern is allocated an embedding bucket.
At the initialization stage, single-edge embeddings
are gather into different single-edge pattern buckets
according to their pattern. Each bucket then is checked
if its support $\sigma$ is above $\sigma_{min}$ by
performing a reduction on the embeddings in its bucket.
If $\sigma < \sigma_{min}$, this pattern is discarded
as well as the entire embedding bucket. During the
\textproc{Extend} phase, each possible new pattern
is allocated a new embedding bucket, and the newly
extended embeddings are then distributed into different
bucket according to its pattern. In this way, the
embeddings of the same pattern are always gathered in
the same embedding bucket, and the pattern reduction can
be simply done by accessing each bucket.

\subsection{Parallelism Issues}
Sandslash is built on top of the Galois~\cite{Galois}
parallel system. Since different worker threads perform
independent DFS walk concurrently, there is no conflict
among threads. Therefore we implement the parallel engine
in \cref{alg:engine} using \texttt{do-all} loops, and let
Galois take control of the parallelization. To balance
the workload for different threads, it relies on the
default work stealing mechanism that Galois provides,
which works well for vertex-induced applications.
For FSM, however, since embeddings are gathered for
each pattern, the stealing unit is a pattern instead
of an embedding. Thus it has relatively coarse-grained
parallelism and is easier to suffer from load imbalance.
Our future work is to enhance the load balancing
mechanism for the case of embedding gathering. 


==> sections/motive.tex <==

\subsection{Limitations of Existing DFS Frameworks}

Fractal~\cite{Fractal} is the first DFS mining system. However, 
it does not support optimizations to avoid redundant computation, 
which is why it is only slightly faster than Arabesque.

AutoMine~\cite{AutoMine} does not support pattern gathering,
which is why it can not use domain support for FSM. Meanwhile,
it automatically generates code from the given paterrn(s) using 
a compiler, therefore application-specific optimizations 
(such as shrinking local graph for $k$-clique and 
formula-based motif counting) are not expressible.
AutoMine may need multiple vertex sets for 5-MC or more.
For multi-pattern, it only keeps one vertex set when
different patterns divergent. Last but not least, since it is over-counting, 
it can only do counting, but not able to do listing.



==> sections/tbl_3fsm.tex <==
\begin{table}[]
\centering
\resizebox{0.46\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc}
\Xhline{2\arrayrulewidth}
\multicolumn{1}{l|}{56-thread} & \multicolumn{3}{c|}{\textbf{Mico}} & \multicolumn{3}{c|}{\textbf{Patent}} & \multicolumn{3}{c}{\textbf{Youtube}} \\ \hline
\textbf{$\sigma$} & \textbf{PR} & \textbf{PA} & \textbf{SA} & \textbf{PR} & \textbf{PA} & \textbf{SA} & \textbf{PR} & \textbf{PA} & \textbf{SA} \\ \hline
\textbf{300}  & 4.4 & 4.2 & 8.9  & 94.2  & 15.9 & 3.4  & 59.3 & 85.2 & 82.5 \\
\textbf{500}  & 4.4 & 3.4 & 9.0  & 103.8 & 17.0 & 3.5  & 52.8 & 86.8 & 81.0 \\
\textbf{1000} & 4.2 & 2.8 & 9.5  & 118.4 & 19.0 & 3.8  & 69.9 & 88.3 & 80.8 \\
\textbf{5000} & 4.3 & 2.3 & 12.5 & 94.3  & 27.4 & 6.1  & 60.8 & 91.5 & 82.8 \\            
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{\small 3-FSM performance of three systems, 
	Peregrine (PR), Pangolin (PA) and Sandslash (SA). 
	$\sigma$: minimum support.}
\label{tab:3-fsm}
\end{table}


\iffalse
\begin{table}[]
	\centering
	\resizebox{0.43\textwidth}{!}{
		\begin{tabular}{c|cc|cc|cc|cc}
			\Xhline{2\arrayrulewidth}
			\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{\tt Mi}} & \multicolumn{2}{c|}{{\tt Pa}} & \multicolumn{2}{c|}{{\tt Yo}} & \multicolumn{2}{c}{{\tt Pdb}} \\ \hline
			\textbf{$\sigma$} & \textbf{PA} & \textbf{SA} & \textbf{PA} & \textbf{SA} & \textbf{PA} & \textbf{SA} & \textbf{PA} & \textbf{SA} \\ \hline
			\textbf{300}  & 4.2 & 8.9  & 15.9 & 3.4  & 86.2 & 82.5 & 54.6  & 44.7  \\
			\textbf{500}  & 3.4 & 9.0  & 17.0 & 3.5  & 86.8 & 81.0 & 57.6  & 46.5  \\
			\textbf{1000} & 2.8 & 9.5  & 19.0 & 3.8  & 88.3 & 80.8 & 66.1  & 40.0  \\
			\textbf{5000} & 2.3 & 12.5 & 27.4 & 6.1  & 91.5 & 82.8 & 117.3 & 44.5  \\            
			\Xhline{2\arrayrulewidth}
		\end{tabular}
	}
	\caption{\small 3-FSM performance (sec) of 
		Pangolin (PA) and Sandslash (SA). 
		$\sigma$: minimum support.}
	\label{tab:3-fsm}
\end{table}

\begin{table}[]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc}
\Xhline{2\arrayrulewidth}
\multicolumn{1}{l|}{} & \multicolumn{3}{c|}{\textbf{Mico}} & \multicolumn{3}{c|}{\textbf{Patent}} & \multicolumn{3}{c}{\textbf{Youtube}} \\ \hline
\textbf{$\sigma$} & \textbf{FR} & \textbf{PA} & \textbf{SA} & \textbf{FR} & \textbf{PA} & \textbf{SA} & \textbf{FR} & \textbf{PA} & \textbf{SA} \\ \hline
\textbf{300}  & 381.9 & 4.2 & 8.9  & 839.2  & 15.9 & 3.4  & - & 85.2 & 82.5 \\
\textbf{500}  & 389.4 & 3.4 & 9.0  & 866.3  & 17.0 & 3.5  & - & 86.8 & 81.0 \\
\textbf{1000} & 385.8 & 2.8 & 9.5  & 1176.2 & 19.0 & 3.8  & - & 88.3 & 80.8 \\
\textbf{5000} & 387.2 & 2.3 & 12.5 & 996.9  & 27.4 & 6.1  & - & 91.5 & 82.8 \\            
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{\small 3-FSM performance of three systems, 
	Fractal (FR), Pangolin (PA) and Sandslash (SA). 
	$\sigma$: minimum support.}
\label{tab:3-fsm}
\end{table}
\fi


==> sections/tbl_4fsm.tex <==
\begin{table}[]
\centering
\footnotesize
\resizebox{0.48\textwidth}{!}{
	\begin{tabular}{c|cccc|cccc}
		\Xhline{2\arrayrulewidth}
		\multicolumn{1}{c|}{56-thread}  & \multicolumn{4}{c|}{{\tt Pa}} & \multicolumn{4}{c}{{\tt Pdb}} \\ \hline
		$\sigma$  & 10K        & 15K        & 20K        & 30K       & 300 & 500 & 1K & 5K\\ \hline
		Sandslash & \bf{102.3} & 110.8      & 108.4      & 43.7      & \bf{189.2} & \bf{200.2} & \bf{198.0} & \bf{195.1} \\
		Pangolin  & -          & 263.9      & 146.2      & 32.7      & - & - & - & - \\
		Peregrine & 28301      & 11527      & 4240.6     & 397.3     & TO & TO & TO & TO \\
		DistGraph & 120.7      & \bf{88.4}  & \bf{58.0} & \bf{25.1} & - & - & - & - \\
		\Xhline{2\arrayrulewidth}
	\end{tabular}%
}
\caption{\small 4-FSM runtime. $\sigma$: 
	minimum support; `-‘: out of memory.}
\label{tab:4-fsm}
\end{table}


==> sections/tbl_esc.tex <==
\begin{table}[]
\centering
%\scriptsize
\resizebox{0.49\textwidth}{!} {
	\begin{tabular}{c|rr|rr|rr|rr|rr|rr}
	\toprule
	                   & \multicolumn{2}{c|}{\textbf{Mi}}  & \multicolumn{2}{c|}{\textbf{Pa}} & \multicolumn{2}{c|}{\textbf{Yo}} & \multicolumn{2}{c|}{\textbf{Lj}} & \multicolumn{2}{c|}{\textbf{Or}} & \multicolumn{2}{c}{\textbf{Fr}} \\ \cline{2-13}
	   & \textbf{CY} & \textbf{DI} & \textbf{CY}  & \textbf{DI} & \textbf{CY}  & \textbf{DI} & \textbf{CY}  & \textbf{DI} & \textbf{CY}  &  \textbf{DI} & \textbf{CY}  & \textbf{DI} \\ \hline
	%\textbf{Fractal}  & 72.0 & 70.8& 447.9 & 871.7& -    & -    \\ %\hline
	%\textbf{AutoMine}  & 2.4 & 0.1 & 1.6 & 0.4 & 10.3 & 0.9 & 174.7 & 2.3 & 2086.7 & 7.4 & 52138.6 & 130.2\\
	%\textbf{Pangolin-old}  & 14.8 & 6.9  & 5.4 & 1.2 & 57.5 & 14.2 & 1191.3 & 333.1 & 23127.9 & 5461.2\\
	\textbf{Pangolin}   & 4.6 & 3.3  & 3.1 & 1.7 & 28.7 & 11.2 & 553.5 & 92.3 & 13208.2 & 884.5 & TO & 9301.6 \\
	\textbf{Peregrine}  & 1.5 & 0.1  & 2.0 & 1.7 & 17.8 & 7.5 & 144.4 & 5.4 & 1867.2 & 10.3 & 32276.8 & \textbf{178.1} \\
	%\textbf{Peregrine (count)}  & 1.3 & 0.05& 1.9 & 0.5 & 17.1 & 1.6 & 139.6 & 2.2 & 1796.7 & 9.1\\
	\textbf{Sandslash-Hi} & \textbf{0.2}  & \textbf{0.04}  & \textbf{0.3} & \textbf{0.3} & \textbf{1.4} & \textbf{0.8}  & \textbf{16.4} & \textbf{1.6} & \textbf{380.1} & \textbf{6.5} & \textbf{20490.9} & 284.2 \\
	\bottomrule
	\end{tabular}
}
\caption{\small Execution time (sec) of SL:- CY: 4-cycle; DI: diamond.}
\label{tab:sl}
\end{table}
\iffalse
\begin{table}[]
	\centering
	%\scriptsize
	\resizebox{0.49\textwidth}{!} {
		\begin{tabular}{c|rrrrrrrr}
			\Xhline{2\arrayrulewidth}
			(sec) & \texttt{Mi} & \texttt{Pa} & \texttt{Yo} & \texttt{Lj} & \texttt{Or} & \texttt{Fr} & \texttt{Tw2} & \texttt{Tw4}\\ \hline
			\textbf{Peregrine} & 0.05 & 0.5 & 1.6 & 2.2 & 8.7 & 158.8 & 245.8 & 16312.6\\
			\textbf{Sandslash} & \textbf{0.03}  & \textbf{0.1} & \textbf{0.4}  & \textbf{0.8} & \textbf{5.8} & \textbf{115.2} & \textbf{194.1} & \textbf{10187.4}\\
			\Xhline{2\arrayrulewidth}
		\end{tabular}
	}
	\caption{\small Subgraph counting on 56 threads. Pattern: {\tt \small diamond}.}
	\label{tab:sc}
\end{table}
\fi

==> sections/tbl_opt_agnostic.tex <==

\begin{table}[]
\centering
\resizebox{0.25\textwidth}{!} {
	\begin{tabular}{c|cccc}
	\Xhline{2\arrayrulewidth}
	  \thead{} & \bf{DF}    & \bf{Mem}   & \bf{MO}    & \bf{DAG}   \\ \hline
		TC     &            &            &            & \checkmark \\
		$k$-CL & \checkmark & \checkmark & \checkmark & \checkmark \\
		SL     & \checkmark & \checkmark & \checkmark &            \\
		$k$-MC &            & \checkmark &            &            \\
		%FSM    &            &            &            &            \\
		\Xhline{2\arrayrulewidth}
		\end{tabular}
	}
	\caption{\small Problem-agnostic optimizations. 
		DF: Degree Filtering;  
		DAG: orientation; 
		MO: Matching Order;
		Mem: Memoization.
	}
	\label{tab:opt_agnostic}
\end{table}


==> sections/tbl_opt_specific.tex <==
\renewcommand\theadalign{bc}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}

\begin{table}[]
	\centering
	\resizebox{0.27\textwidth}{!}{
		\begin{tabular}{c|ccccc}
			\Xhline{2\arrayrulewidth}
			        & \bf{FP}    & \bf{CP}    & \bf{LG}    & \bf{LC}    & \thead{PF}\\ \hline
			TC      & \checkmark & \checkmark &            &            &           \\
			$k$-CL  & \checkmark & \checkmark & \checkmark &            &           \\
			SL      & \checkmark & \checkmark &            &            &           \\
			$k$-MC  & \checkmark & \checkmark &            & \checkmark &           \\
			$k$-FSM &            & \checkmark &            &            & \checkmark\\
			\Xhline{2\arrayrulewidth}
		\end{tabular}
	}
	\caption{\small Problem-specific optimizations.
		FP: Fine-grained Pruning;
		CPC: Customized Pattern Classification; 
		LG: search on Local Graph; 
		LC: Local Counting;
		PF: Pattern Filtering. }
	\label{tab:opt}
\end{table}



==> sections/tbl_sys_exp.tex <==
\begin{table}[]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|cccccc}
\Xhline{2\arrayrulewidth}
          &  \begin{tabular}[c]{@{}l@{}}Vertex\\ Induced\end{tabular} &\begin{tabular}[c]{@{}l@{}}Edge\\ Induced\end{tabular}& Listing & \begin{tabular}[c]{@{}l@{}}Explicit\\ Patterns\end{tabular}  &  \begin{tabular}[c]{@{}l@{}}Implicit\\ Patterns\end{tabular} & \begin{tabular}[c]{@{}l@{}}Custom\\ Support\end{tabular}\\ \hline
Arabesque~\cite{Arabesque} & \checkmark & \checkmark & \checkmark &\checkmark &\checkmark  & \checkmark \\
RStream~\cite{RStream}     & \checkmark & \checkmark & \checkmark &\checkmark & \checkmark &            \\
Fractal~\cite{Fractal}     & \checkmark & \checkmark & \checkmark &\checkmark & \checkmark & \checkmark \\
Pangolin~\cite{Pangolin}   & \checkmark & \checkmark & \checkmark &\checkmark & \checkmark & \checkmark \\
AutoMine~\cite{AutoMine}   & \checkmark &            &            &\checkmark & \checkmark &            \\
%GraphZero~\cite{GraphZero} & \checkmark &            & \checkmark &\checkmark &            &            \\
Peregrine~\cite{Peregrine} & \checkmark & \checkmark & \checkmark &\checkmark & \checkmark & \checkmark \\
Sandslash                  & \checkmark & \checkmark & \checkmark &\checkmark & \checkmark & \checkmark \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{\small Expressiveness of GPM systems.}
\label{tab:sys_exp}
\end{table}





\iffalse{
\begin{table}[]
    \centering
    % \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|ccccc}
    \Xhline{2\arrayrulewidth}
              & Subgraph Type & Listing/Counting & Matching/Mining   & Domain support & Exploration \\ \hline
    Arabesque & V + E         & L + C            & Matching + Mining & Y              & BFS         \\
    RStream   & E             & L + C            & Matching + Mining & N              & BFS         \\
    Fractal   & V + E         & L + C            & Matching + Mining & Y              & DFS         \\
    Pangolin  & V + E         & L + C            & Matching + Mining & Y              & BFS         \\
    AutoMine  & V + E         & C                & Matching + Mining & N              & DFS         \\
    GraphZero & V             & L + C            & Matching          & N              & DFS         \\
    Peregrine & V + E         & L + C            & Matching + Mining & Y              & DFS         \\
    Sandslash & V + E         & L + C            & Matching + Mining & Y              & DFS         \\
    \Xhline{2\arrayrulewidth}
    \end{tabular}
    % }
    \caption{Comparing expressiveness of different systems.}
    \label{tab:sys_exp}
    \end{table}
}\fi


==> sections/tbl_sys_kcl.tex <==
\begin{table}[t]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|rrrr|rrrr}
	\Xhline{2\arrayrulewidth}
28-thread          & \multicolumn{4}{c|}{\textbf{4-CL}}  & \multicolumn{4}{c}{\textbf{5-CL}} \\ \hline
(sec)              & \textbf{Mi} & \textbf{Pa} & \textbf{Lj} & \textbf{Or} & \textbf{Mi} & \textbf{Pa} & \textbf{Lj} & \textbf{Or} \\ \hline
%\textbf{Sandslash-Lo} & 0.17 & 0.13 & 2.7& 4.8  & 3.5   & 0.14 & 71.7   & 14.4  \\
%\textbf{Sandslash-Hi} & 0.13 & 0.2  & 2.2& 6.9  & 4.5   & 0.2  & 74.3   & 41.1  \\
\textbf{AutoMine}     & -    & -    & -    & -   & 11.4& 0.17 & -     & -   \\
\textbf{Pangolin}     & 1.6  & 0.4  & 26.3 & 82.3& 60.5& 0.5  & 1914.1& 422.3 \\
\textbf{Peregrin}     & 0.9  & 0.7  & 26.1 &130.9& 28.7& 0.8  & 931.2 & 1402.0  \\
\textbf{Sandslash-Hi} & \textbf{0.06} & 0.15 & \textbf{1.2}  & 4.6 & \textbf{1.6} & 0.14 & \textbf{27.6}  & 14.5 \\
\textbf{Sandslash-Lo} & 0.1  & \textbf{0.08} & 1.6  & \textbf{4.3} & 2.2 & \textbf{0.08} & 27.8  & \textbf{10.6} \\
\Xhline{2\arrayrulewidth}     
\end{tabular}
}
\caption{\small $k$-CL runtime on 28 threads. `-': not available.}
\label{tab:sys-kcl}
\end{table}
%\textbf{Fractal}   & 47.9 & 225.6 & -    & -    & 355.1 & 258.6& -      & -     \\


==> sections/tbl_sys_kmc.tex <==
\begin{table}[t]
\centering
\resizebox{0.48\textwidth}{!} {
\begin{tabular}{c|rrrr|rrrr}
\Xhline{2\arrayrulewidth}
28-thread          & \multicolumn{4}{c|}{\textbf{3-MC}} & \multicolumn{4}{c}{\textbf{4-MC}}\\ \hline
(sec)              & \textbf{Mi} & \textbf{Pa} & \textbf{Lj} & \textbf{Or} & \textbf{Mi} & \textbf{Pa} & \textbf{Lj} & \textbf{Or} \\ \hline
\textbf{AutoMine}  & 0.23 & 1.9  & 13.4 & 82.2  & 45.2  & 82.1  & 22020.0 & 157320.0 \\
\textbf{Pangolin}  & 0.2  & 0.9  & 19.5 & 176.3 & 175.6 & 209.1 & TO    & TO     \\
\textbf{Peregrin}  & 0.08 & 1.4  & 3.0  & \textbf{7.9}   & 6.3   & 11.0  & 285.4 & 3037.0   \\
\textbf{Sandslash-Hi} & 0.06 & 0.4 & 3.3& 20.0  & 9.5   & 8.6   & 3987.0  & 58331  \\
\textbf{Sandslash-Lo} & \textbf{0.03} & \textbf{0.2} & \textbf{1.8}& 12.2  & \textbf{2.5}   & \textbf{2.9}   & \textbf{127.9}   & \textbf{1611.9}   \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{\small $k$-MC performance on 28 threads. TO: timed out.}
\label{tab:sys-kmc}
\end{table}
%\textbf{GraphZero} & 0.06 & 0.74 & 4.02 & 23.1  & 15.2  & 10.2  & 3240  & 26640  \\
%\textbf{Fractal}   & 45.2 & 429.6& -    & -     & 165.8 & 485.9 & -     & -      \\


==> sections/tbl_sys_opt.tex <==
\def\semichecked{\checkmark\!\!\!\raisebox{0.4 em}{\tiny$\smallsetminus$}}

\begin{table}[t]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|ccccc|cccc}
\Xhline{2\arrayrulewidth}
\multicolumn{1}{l|}{} & \multicolumn{5}{c|}{\textbf{High-level Optimizations}}                         & \multicolumn{4}{c}{\textbf{Low-level Optimizations}} \\ \hline
\multicolumn{1}{l|}{} & SB         & DAG        & MO         & \textbf{DF}& \textbf{Mem} & FP          & CP          & \textbf{LG} & \textbf{LC}\\ \hline %& PF         
\textbf{AutoMine}     &            &            & \checkmark &            & $\circledcirc$ &             &             &             &            \\        %&            
\textbf{Pangolin}     & \checkmark & \checkmark & \checkmark &            & $\circledcirc$ & \checkmark  & \checkmark  &             &            \\        %&            
\textbf{Peregrine}    & \checkmark &            & \checkmark &            & $\circledcirc$ &             &             &             &            \\        %&            
\textbf{SS-Hi}        & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark   &             &             &             &            \\        %& \checkmark 
\textbf{SS-Lo}        & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark   & \checkmark  & \checkmark  & \checkmark  & \checkmark \\        %& \checkmark 
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{Optimizations enabled in different frameworks. 
  $\checkmark$: fully supported; $\circledcirc$: limited support.}
\label{tab:sys_opt}
\end{table}


==> sections/tbl_systems.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
	\centering
	\footnotesize
	\resizebox{0.95\textwidth}{!}{%
	\begin{tabular}{l|c|rrrr|rrrr|rrrr}
		\hline
		\multicolumn{2}{c|}{Inputs}   & \multicolumn{4}{c|}{Mico} & \multicolumn{4}{c|}{Patent}  & \multicolumn{4}{c}{Youtube}   \\ \hline
		Apps & \multicolumn{1}{l|}{Options} & 
		\multicolumn{1}{c}{AR} & \multicolumn{1}{c}{RS} & \multicolumn{1}{c}{FR} & \multicolumn{1}{c|}{SA} & 
		\multicolumn{1}{c}{AR} & \multicolumn{1}{c}{RS} & \multicolumn{1}{c}{FR} & \multicolumn{1}{c|}{SA} & 
		\multicolumn{1}{c}{AR} & \multicolumn{1}{c}{RS} & \multicolumn{1}{c}{FR} & \multicolumn{1}{c}{SA}\\ \hline
		\multirow{4}{*}{3-FSM} & 300 & 120.2 & 102.3 & 381.8 & 9.7 & 393.6 & 364.0 & 839.2 & 5.12 & - & 1670.9 & - & 86.7 \\
		& 500  & 88.1  & 94.0 & 389.4  & 9.3 & 446.5  & 352.9  & 866.3  & 5.6 & -   & 1685.7  & -   & 86.5  \\
		& 1000 & 58.1  & 88.3 & 385.8  & 9.9 & 425.9  & 329.4  & 1176.2  & 6.6  & -  & 1560.9   & - & 84.6  \\
		& 5000 & 41.2  & 80.0 & 387.2 & 13.2 & 433.9  & 315.9 & 996.9  & 11.8 & - & 1566.8  & -  & 86.6 \\ \hline
		\multirow{2}{*}{MC} & 3 & 37.1  & 7265.3  & 45.2  & 0.02 & 119.4 & 4404.2 & 429.6 & 0.3 & 949.0   & 90674.8 & - & 0.9  \\
							& 4 & 261.1 & -       & 165.8 & 1.4  & 750.9 & -      & 485.9 & 1.8 & 90348.4 & -       & - & 12.2 \\ \hline
		\multirow{2}{*}{CL} 
		%& 3  & 36.2  & 14.0   & 48.5  & 0.01 & 121.9& 45.5 & 234.4 & 0.1   & 1019.2 & 2236.3&-& 0.3\\
		& 4  & 45.2  & 1391.2 & 49.9  & 0.1  & 132.7& 81.4 & 235.2 & 0.1   & 1304.9 & -  & -  & 0.4  \\
		& 5  & 223.7 & -      & 222.8 & 1.9  & 139.9& 91.2 & 245.6 & 0.1   & 1619.1 & -  & -  & 0.5 \\ \hline
		TC & & 35.9  & 2.8 &  &  0.01 & 127.0& 5.9  &      & 0.04  & 1077.7& 36.3   &    & 0.2   \\ \hline
		\end{tabular}%
	}
	\caption{Comparing Sandslash (SA) runtime (sec) with existing mining systems 
    Arabesque (AR), RStream (RS), Fractal (FR). Option: minimum support for 3-FSM; 
    $k$ for other applications. `-' indicates out of memory or disk, or timed out in 30 hours.}
	\label{tab:systems}
\end{table*}


==> sections/tbl_vsc.tex <==
\begin{table}[]
\centering
\resizebox{0.22\textwidth}{!} {
	\begin{tabular}{c|ccc}
	\Xhline{2\arrayrulewidth}
	28-thread& \textbf{\tt Mi} & \textbf{\tt Pa} & \textbf{\tt Lj} \\ \hline
	\textbf{Sandslash} & 1.3 & 2.5 & 105.6 \\
	\textbf{AutoMine}  & 6   & 15  & 900   \\
	%\textbf{GraphZero} & 0.5 & 1.1 & 80    \\
	%\textbf{Peregrine} & 0.5 & 1.1 & 80    \\
	\Xhline{2\arrayrulewidth}             
	\end{tabular}
}
\caption{\small V-SL performance (pattern: 4-cycle). }
\label{tab:vsc}
\end{table}

